Connecting orbits for a singular nonautonomous real Ginzburg-Landau type equation

We propose a method for computation of stable and unstable sets associated to hyperbolic equilibria of nonautonomous ODEs and for computation of specific type of connecting orbits in nonautonomous singular ODEs. We apply the method to a certain a singular nonautonomous real Ginzburg-Landau type equation, which that arises from the problem of formation of spots in the Swift-Hohenberg equation.

==> shoot-geo.tex <==
\section{Shooting between manifolds}
\label{sec:shooting}


\textbf{PZ: nie jest dla mnie jasne czy to powinien byc osobny rozdzial, czy jakos nie zlac go z nastepnym - albo tam jako podrozdzial. Lub wyrzucic}

Given isolating blocks with cone condition we can express the local unstable and stable sets as graphs of functions. Using an ODE solver one can integrate forward in time a slice of unstable manifold and check whether it intersect the stable manifold. This problem can be transformed to zero finding problem of a~certain function that is built on the local parameterizations of invariant manifold and some Poincar\'e map.

Our shooting parameter will be the initial time $r$ on the upper exit face of $\Nbeg$ obtained in Section~\ref{sec:unstb-man-beg}. Let $\Nbeg$ and $\Nend$ be isolating blocks for $r\to 0$ and $r\to \infty$, respectively.

Since to treat $r \to 0$ we did the substitution $\rho=\ln r$, we should be careful with symbols $A'$ and $w'$. We have  $A'(r)=\frac{d A}{dr}$, while $w'=w'(\rho)=\frac{d w}{d \rho}$. Differentiating $A(r)=w(\rho(r))$ we obtain
\begin{equation*}
  A'(r)=\frac{w'(\rho(r))}{r}.
\end{equation*}

Let us denote by $C$ the following map
\begin{equation*}
  C(r,w,w')=(r,w,w'/r)
\end{equation*}
which realizes the change of the 'time' variable.

We define two Poincar\'e sections
\begin{itemize}
\item $\Pibeg$ - the starting section, which is the upper
exit face of $\Nbeg=[-\dbeg_1,\dbeg_1]\times[-\dbeg_2,\dbeg_2]$ obtained in Section~\ref{sec:unstb-man-beg}. It is used for equation (\ref{eq:sing-r=0}) and in variables $(\rho,w,w')$ it is given by
$(w+2w')/2=\dbeg_1$. In terms of original variables $(r,A,A')$,
this equation becomes
\begin{equation*}
  \frac{A+ 2rA'}{2}=\dbeg_1.
\end{equation*}
\item $\Piend$ - the section for $r\to\infty$. It is given by lower $\Nend=[-\dend_1,\dend_1]\times[-\dend_2,\dend_2]$
edge , i.e. $\yend=-\dend_2$, which in the original coordinates is given by relation
\begin{equation*}
  A - A'=-\dend_2.
\end{equation*}
\end{itemize}


Assuming the cone conditions are satisfied on $\Nbeg$ and $\Nend$ the local unstable and stable sets can be expressed as graphs of smooth functions
\begin{eqnarray*}
W^u_{\rho,\Nbeg}(0)&=&\{(\xbeg,\ybeg(\rho,\xbeg)) \ | \ \xbeg \in
[-\dbeg_1,\dbeg_1]\},\\
W^s_{r,\Nend}(0)&=&\{(\xend(r,y),\yend) \ | \ \yend
\in [-\dend_2,\dend_2]\}.
\end{eqnarray*}
and we have the bounds for their first order derivatives.


Let $P: \Pibeg\to\Piend$ be the Poincar\'e map. For $(r_0,A_0,A_0')\in\Pibeg$ the point $(r,A,A')=P(r_0,A_0,A_0')$ is the first intersection of the forward trajectory of $(r_0,A_0,A_0')$ with $\Piend$ provided it exists. Clearly, the mapping $P$ is well defined in some vicinity of connecting orbit we are looking for.

Let $\Tbeg$ be the linear transformation, which maps the 'good' coordinates in $\Nbeg$ to the standard ones. It is given by (compare (\ref{eq:gc-n-in}))
\begin{equation*}
  \Tbeg(r,\xbeg,\ybeg)=(r,w,w')=\left(r,\xbeg+\ybeg,\frac{\xbeg-\ybeg}{2}\right).
\end{equation*}

Let $\Tend$ be the linear transformation, which maps the standard coordinates to the good ones in $\Nend$ and it is given by (compare (\ref{eq:gc-n-out-inv}))
\begin{equation*}
  \Tend(r,A,A')=(r,\xend,\yend) = (r,A+A',A-A').
\end{equation*}


\textbf{PZ: Tego ponizej nie da sie zrozumiec:}
To realize the shooting we have to prove that the following map \textbf{(in fact a composition of three maps)} has zero
\begin{multline*}
   \mathbb{R} \ni \rbeg \mapsto (\rbeg,A(\rbeg),A(\rbeg)'):=(C\circ \Tbeg)\left(\rbeg,\dbeg_1,\ybeg(\ln \rbeg,\dbeg_1)\right) \mapsto \\ 		
   (\rend,A_\mend,A'_\mend):=P\left(\rbeg,A(\rbeg),A(\rbeg)'\right) \mapsto \\
   (\rend,\xend,\yend) := \Tend(\rend,A_\mend,A'_\mend) \mapsto
     \xend - \xend(\rend,-\dend_2) \in \mathbb{R}.
\end{multline*}





==> shooting.tex <==
\section{The shooting method}

The software for the rigorous integration for ODEs (for example CAPD) exists, so there
is not a problem in obtaining  bounds of good quality for behavior of solutions of ODEs
on reasonably long, but finite, time intervals. However in the present problem the infinite
time interval has to be considered.

Therefore to realize the shooting method for (\ref{eq:MS}) one needs to deal with
the following issues
\begin{description}
\item[1] the singularity for $r=0$
\item[2] since the equation is non-autonomous the standard tools for the estimates of the
stable manifold of the point $(A,A')=(0,0)$ does not apply
\end{description}
Issue 1 is dealt with via the change of the independent variable $\rho=\ln r$.
The equation (\ref{eq:MS}) becomes
\begin{equation}
  w" - w/4 = e^{2\rho}(w-w^3).  \label{eq:sing-r=0}
\end{equation}
 Now we seek a solution such that $\lim_{\rho\to -\infty} w(\rho)=0$, so we need estimates
 for the unstable set of $(w=0,w'=0)$ for $\rho \to -\infty$ for our non-autonomous ODE
 (\ref{eq:sing-r=0}), which is basically issue 2 above.

Rigorous bounds for the stable and unstable manifolds for fixed
point for nonautonomous ODEs can be  obtained by adapting the
methods of cones for ODEs in the present context. The computations
by pen and pencil show we can estimate these sets in our problem
up to the distance $0.1$ from the origin. This will be show in the
following sections. This is a good news, because the time interval
for which we would like to obtain rigorous bounds for the
integration will be not to long.


\section{Notation}
For a matrix $A \in \mathbb{R}^{n \times k}$ by $A^T$ we will
denote its transpose.

For the bilinear map $M:V \times W \to \mathbb{R}$ we will use the
norm $\|W\|=\max_{\|v\|\leq 1, \|w\| \leq 1 } |M(v,w)|$.

